Homogeneous structures and rigidity of isoparametric submanifolds in Hilbert space

We study isoparametric submanifolds of rank at least two in a separable Hilbert space, which are known to be homogeneous by a result of Heintze and Liu, and associate to such a submanifold M and a point x in M a canonical homogeneous structure (a certain bilinear map on the tangent space). We prove that the homogeneous structure together with the second fundamental form encodes all the information about M, and deduce from this the rigidity result that M is completely determined by the second fundamental form and its covariant derivative, thereby making such submanifolds accessible to classification. As an essential step, we show that the one-parameter groups of isometries constructed by Heintze and Liu to prove their homogeneity induce smooth and hence everywhere defined Killing fields, implying the continuity of the homogeneous structure. Here an important tool is the introduction of affine root systems of isoparametric submanifolds.

==> BCn_30.tex <==
\setlength{\unitlength}{1184sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup

\newcommand{\BCn}[4]{
\begin{picture}(5152,895)(1025,-4136)
\thinlines
\put(1201,-3961){\circle{336}}
\put(2401,-3961){\circle{336}}
\put(4801,-3961){\circle{336}}
\put(6001,-3961){\circle{336}}
\put(3436,-3946){\circle*{30}}
\put(3586,-3946){\circle*{30}}
\put(3736,-3946){\circle*{30}}
\put(1369,-3961){\line( 1, 0){864}}
\put(2569,-3961){\line( 1, 0){600}}
\put(4003,-3961){\line( 1, 0){600}}
\put(4969,-3911){\line( 1, 0){864}}
\put(4969,-4011){\line( 1, 0){864}}
\put(1141,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#1$}}}}
\put(2341,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#2$}}}}
\put(4741,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#3$}}}}
\put(5941,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#4$}}}}
\end{picture}
}

==> Bn1_30.tex <==
\setlength{\unitlength}{1184sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup

\newcommand{\Bni}[5]{
\begin{picture}(6352,895)(1025,-4136)
\thinlines
\put(1201,-3961){\circle{336}}
\put(2401,-3961){\circle{336}}
\put(3601,-3961){\circle{336}}
\put(6001,-3961){\circle{336}}
\put(7201,-3961){\circle*{336}}

\put(1369,-3961){\line( 1, 0){864}}
\put(2569,-3961){\line( 1, 0){864}}
\put(3769,-3961){\line( 1, 0){600}}
\put(5203,-3961){\line( 1, 0){600}}
\put(6169,-3911){\line( 1, 0){864}}
\put(6169,-4011){\line( 1, 0){864}}

\put(4636,-3946){\circle*{30}}
\put(4786,-3946){\circle*{30}}
\put(4936,-3946){\circle*{30}}

\put(1141,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#1$}}}}
\put(2341,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#2$}}}}
\put(3541,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#3$}}}}
\put(5941,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#4$}}}}
\put(7141,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#5$}}}}

\end{picture}
}

==> Bn2_30.tex <==
\setlength{\unitlength}{1184sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup

\newcommand{\Bnii}[6]{
\begin{picture}(7552,895)(1025,-4136)
\thinlines
\put(1201,-3961){\circle{336}}
\put(2401,-3961){\circle{336}}
\put(3601,-3961){\circle{336}}
\put(4801,-3961){\circle{336}}
\put(7201,-3961){\circle{336}}
\put(8401,-3961){\circle*{336}}

\put(1369,-3961){\line( 1, 0){864}}
\put(2569,-3961){\line( 1, 0){864}}
\put(3769,-3961){\line( 1, 0){864}}

\put(4903,-3961){\line( 1, 0){600}}
\put(6403,-3961){\line( 1, 0){600}}
\put(7369,-3911){\line( 1, 0){864}}
\put(7369,-4011){\line( 1, 0){864}}

\put(5836,-3946){\circle*{30}}
\put(5986,-3946){\circle*{30}}
\put(6136,-3946){\circle*{30}}

\put(1141,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#1$}}}}
\put(2341,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#2$}}}}
\put(3541,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#3$}}}}
\put(4741,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#4$}}}}
\put(7141,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#5$}}}}
\put(8341,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#6$}}}}

\end{picture}
}

==> Bn3_30.tex <==
\setlength{\unitlength}{1184sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup

\newcommand{\Bniii}[7]{
\begin{picture}(8752,895)(1025,-4136)
\thinlines
\put(1201,-3961){\circle{336}}
\put(2401,-3961){\circle{336}}
\put(3601,-3961){\circle{336}}
\put(4801,-3961){\circle{336}}
\put(7201,-3961){\circle{336}}
\put(8401,-3961){\circle{336}}
\put(9601,-3961){\circle*{336}}

\put(1369,-3961){\line( 1, 0){864}}
\put(2569,-3961){\line( 1, 0){864}}
\put(3769,-3961){\line( 1, 0){864}}

\put(4903,-3961){\line( 1, 0){600}}
\put(6403,-3961){\line( 1, 0){600}}

\put(7369,-3961){\line( 1, 0){864}}

\put(8569,-3911){\line( 1, 0){864}}
\put(8569,-4011){\line( 1, 0){864}}

\put(5836,-3946){\circle*{30}}
\put(5986,-3946){\circle*{30}}
\put(6136,-3946){\circle*{30}}

\put(1141,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#1$}}}}
\put(2341,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#2$}}}}
\put(3541,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#3$}}}}
\put(4741,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#4$}}}}
\put(7141,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#5$}}}}
\put(8341,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#6$}}}}
\put(9541,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#7$}}}}

\end{picture}
}

==> Bns_30.tex <==
\setlength{\unitlength}{1184sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup

\newcommand{\Bns}[3]{
\begin{picture}(3952,895)(1025,-4136)
\thinlines
\put(1201,-3961){\circle{336}}
\put(3601,-3961){\circle{336}}
\put(4801,-3961){\circle*{336}}
\put(2236,-3946){\circle*{30}}
\put(2386,-3946){\circle*{30}}
\put(2536,-3946){\circle*{30}}
\put(1369,-3961){\line( 1, 0){600}}
\put(2803,-3961){\line( 1, 0){600}}
\put(3769,-3911){\line( 1, 0){864}}
\put(3769,-4011){\line( 1, 0){864}}
\put(1141,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#1$}}}}
\put(3541,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#2$}}}}
\put(4741,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#3$}}}}
\end{picture}
}

==> Bntb_30.tex <==
\setlength{\unitlength}{1184sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup

\newcommand{\Bntb}[5]{
\begin{picture}(5151,2200)(1123,-4136)
\thinlines
\put(1549,-3109){\circle{336}}
\put(1549,-4813){\circle{336}}
\put(2401,-3961){\circle{336}}
\put(4801,-3961){\circle{336}}
\put(6001,-3961){\circle*{336}}
\put(3436,-3946){\circle*{30}}
\put(3586,-3946){\circle*{30}}
\put(3736,-3946){\circle*{30}}
\put(1667,-3227){\line( 1, -1){615}}
\put(1667,-4695){\line( 1, 1){615}}
\put(2569,-3961){\line( 1, 0){600}}
\put(4003,-3961){\line( 1, 0){600}}
\put(4969,-3911){\line( 1, 0){864}}
\put(4969,-4011){\line( 1, 0){864}}
\put(926,-3211){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#1$}}}}
\put(926,-4936){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#2$}}}}
\put(2341,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#3$}}}}
\put(4741,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#4$}}}}
\put(5941,-3436){\makebox(0,0)[lb]{\smash{\SetFigFont{6}{7.2}{rm}\mbox{$#5$}}}}
\end{picture}
}

==> macros.tex <==
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{array}
\usepackage{multirow}
%\usepackage{graphicx}
%\usepackage{amscd}
\usepackage[small,nohug%,heads=littlevee
]{diagrams}
%\diagramstyle[labelstyle=scriptstyle]
%\usepackage{theorem}

\input{A7_30.tex}
\input{A6_30.tex}
\input{A5_30.tex}
\input{A4_30.tex}
\input{A3_30.tex}
\input{A2_30.tex}
\input{A2t_30.tex}
\input{A1_30.tex}

\input{B8_30.tex}
\input{B7_30.tex}
\input{B6_30.tex}
\input{B5_30.tex}
\input{B4_30.tex}
\input{B3_30.tex}
\input{B3t_30.tex}
\input{B2_30.tex}

\input{C8_30.tex}
\input{C7_30.tex}
\input{C6_30.tex}
\input{C5_30.tex}
\input{C4_30.tex}
\input{C3_30.tex}
\input{C3t_30.tex}
\input{C2_30.tex}
\input{C2t_30.tex}
\input{C2tb_30.tex}
\input{C2ta_30.tex}
\input{C2tar_30.tex}
\input{C2ta2_30.tex}
\input{C2ta3_30.tex}



\input{D9_30.tex}
\input{D8_30.tex}
\input{D7_30.tex}
\input{D6_30.tex}
\input{D5_30.tex}
\input{D4_30.tex}

\input{F4_30.tex}
\input{F4e_30.tex}
\input{F4t_30.tex}
\input{F4tb_30.tex}
\input{G2_30.tex}
\input{G2e_30.tex}
\input{G2t_30.tex}
\input{G2tb_30.tex}
\input{E6_30.tex}
\input{E6t_30.tex}
\input{E7_30.tex}
\input{E7t_30.tex}
\input{E8_30.tex}
\input{E8t_30.tex}

\input{An_30.tex}
\input{Anl_30.tex}
\input{Ans_30.tex}
\input{An1_30.tex}
\input{An2_30.tex}
\input{An3_30.tex}
\input{Ant_30.tex}
\input{Bn_30.tex}
\input{Bns_30.tex}
\input{Bn1_30.tex}
\input{Bn2_30.tex}
\input{Bn3_30.tex}
\input{Bn4_30.tex}
\input{Bnt_30.tex}
\input{Bntb_30.tex}
\input{Bnta_30.tex}
\input{BC2_30.tex}
\input{BC3_30.tex}
\input{BC4_30.tex}
\input{BCn_30.tex}
\input{Cn_30.tex}
\input{Cns_30.tex}
\input{Cnt_30.tex}
\input{Cntb_30.tex}
\input{Cnta_30.tex}
\input{Cnta2_30.tex}
\input{Cnta3_30.tex}
\input{Cntar_30.tex}
\input{Cntar2_30.tex}
\input{Cntar3_30.tex}
\input{Cn1_30.tex}
\input{Cn2_30.tex}
\input{Dn_30.tex}
\input{Dns_30.tex}
\input{Dnt_30.tex}
\input{Dn1_30.tex}
\input{Dn2_30.tex}
\input{Dn3_30.tex}
\input{Dn4_30.tex}




\flushbottom
%\renewcommand{\baselinestretch}{1.5}
\topmargin 0pt
\headheight 0pt
\headsep 0pt
\oddsidemargin 0pt
\evensidemargin 0pt
\textheight 9in
\textwidth 6.5in
%\addtolength{\footskip}{.2in}



\newcommand{\Lg}{\mbox{$\mathfrak g$}}
\newcommand{\Ll}{\mbox{$\mathfrak l$}}
\newcommand{\Lh}{\mbox{$\mathfrak h$}}
\newcommand{\Lk}{\mbox{$\mathfrak k$}}
\newcommand{\Lp}{\mbox{$\mathfrak p$}}
\newcommand{\La}{\mbox{$\mathfrak a$}}
\newcommand{\Lm}{\mbox{$\mathfrak m$}}
\newcommand{\Ln}{\mbox{$\mathfrak n$}}
\newcommand{\Lc}{\mbox{$\mathfrak c$}}
\newcommand{\Lt}{\mbox{$\mathfrak t$}}
\newcommand{\Lq}{\mbox{$\mathfrak q$}}
\newcommand{\Ls}{\mbox{$\mathfrak s$}}
\newcommand{\Lz}{\mbox{$\mathfrak z$}}
\newcommand{\Lso}{\mbox{$\mathfrak so$}}

\newcommand{\D}{\mbox{$\mathcal D$}}

\newcommand{\Pf}{{\em Proof}. }
\newcommand{\EPf}{\hfill$\square$}
\newcommand{\Z}{\mbox{$\mathbf Z$}}
\newcommand{\R}{\mbox{$\mathbf R$}}
\newcommand{\C}{\mbox{$\mathbf C$}}
\newcommand{\Q}{\mbox{$\mathbf H$}}

\newcommand{\inn}[2]{\mbox{$\mathcal{h} #1,#2 \mathcal{i}$}}
\newcommand{\ad}[1]{\mbox{$\mbox{ad}_{#1}$}}
\newcommand{\Ad}[1]{\mbox{$\mbox{Ad}_{#1}$}}
\newcommand{\Exp}{\mbox{$\mbox{Exp}$}}
\newcommand{\ontop}[2]{\genfrac{}{}{0pt}{}{#1}{#2}}
\newcommand{\tr}{\mbox{$\mbox{trace}$}}
\newcommand{\scalar}[2]{\mbox{$\mathcal{h} #1,#2 \mathcal{i}$}}
\newcommand{\tp}{\mbox{$\tilde p$}}
\newcommand{\tN}{\mbox{$\tilde N$}}

\newcommand{\SU}[1]{\mbox{$\mathbf{SU}(#1)$}}
\newcommand{\U}[1]{\mbox{$\mathbf{U}(#1)$}}
\newcommand{\SP}[1]{\mbox{$\mathbf{Sp}(#1)$}}
\newcommand{\SO}[1]{\mbox{$\mathbf{SO}(#1)$}}
\newcommand{\OG}[1]{\mbox{$\mathbf{O}(#1)$}}
\newcommand{\Spin}[1]{\mbox{$\mathbf{Spin}(#1)$}}
\newcommand{\F}{\mbox{$\mathbf{F}_4$}}
\newcommand{\G}{\mbox{$\mathbf{G}_2$}}



\pagestyle{plain}
%\theoremstyle{change}
%\theorembodyfont{\itshape}

%\swapnumbers
\newtheorem{thm}[equation]{Theorem}
\newtheorem{dfn}[equation]{Definition}
\newtheorem{rmk}[equation]{Remark}
\newtheorem{cor}[equation]{Corollary}
\newtheorem{prop}[equation]{Proposition}
\newtheorem{lem}[equation]{Lemma}
\newtheorem{exs}[equation]{Examples}
\newtheorem{conj}[equation]{Conjecture}

%\newtheorem{thm}{Theorem}[section]
%\newtheorem{dfn}{Definition}[section]
%\newtheorem{rmk}{Remark}[section]
%\newtheorem{cor}{Corollary}[section]
%\newtheorem{prop}{Proposition}[section]
%\newtheorem{lem}{Lemma}[section]
%\newtheorem{exs}{Examples}[section]
%\newtheorem{conj}{Conjecture}[section]




\theoremstyle{remark}
\newtheorem{rem}[equation]{Remark}%[section]

\theoremstyle{remark}
\newtheorem{defn}[equation]{Definition}%[section]


\renewcommand{\theequation}{\thesection.\arabic{equation}}
\renewcommand{\thethm}{\thesection.\arabic{thm}}
\renewcommand{\theenumi}{\(\alph{enumi}\)}

%\renewcommand{\thefootnote}{$\blacksquare$\arabic{footnote}$\blacksquare$}
\newcommand{\ft}{\footnote}

